Towards Automatic Detection of Misinformation in Online Medical Videos

Recent years have witnessed a significant increase in the online sharing of medical information, with videos representing a large fraction of such online sources. Previous studies have however shown that more than half of the health-related videos on platforms such as YouTube contain misleading information and biases. Hence, it is crucial to build computational tools that can help evaluate the quality of these videos so that users can obtain accurate information to help inform their decisions. In this study, we focus on the automatic detection of misinformation in YouTube videos. We select prostate cancer videos as our entry point to tackle this problem. The contribution of this paper is twofold. First, we introduce a new dataset consisting of 250 videos related to prostate cancer manually annotated for misinformation. Second, we explore the use of linguistic, acoustic, and user engagement features for the development of classification models to identify misinformation. Using a series of ablation experiments, we show that we can build automatic models with accuracies of up to 74%, corresponding to a 76.5% precision and 73.2% recall for misinformative instances.

==> rebuttal.tex <==

Thanks to the reviewers for their valuable feedback. Please see below our responses to the main points raised in the reviews. 

R1

- We will replace the accuracy metric with error reduction rate so it reflects more accurately the performance gain while using the proposed method. 

- In addition to reporting accuracy, we will report precision, recall, and f-score on individual classes, so they reflect more accurately the per-class performance. 

- We selected an SVM classifier due to the limited number of examples and the large number of features. SVM classifiers have shown good performance in multimodal tasks in the past. We did try other algorithms, however they did not perform better than the SVM classifier. In addition, due to the limited training data we were unable to apply successfully a deep learning based model.

- About 40\% of the videos in our dataset have two speakers. These videos mainly consist of interviews with doctors and patients.

R3
- The main difference between our work and the study presented in Ref.1 is that Ref.1 only presents descriptive and statistical analyses of the content of videos discussing prostate cancer, which mainly revealed the increasing presence of misinformative content. Instead, we present a data-driven approach to build learning models able to distinguish between trustworthy and misinformative content in prostate cancer videos.

- We believe our method will generalize well to the large number of videos that have the same properties as the videos in our dataset. Methodological changes may be required for videos that have different characteristics (e.g., vlogs with voice layover; videos including a large number of people). Our future research will consider expanding our data collection to analyze a larger sample and confirm our findings. 

- The filtering process for the videos included in our dataset is mainly based on methodologies used in previous work when performing content analysis of prostate cancer videos (e.g., see Ref.1). As mentioned in the discussion section, we agree that some of the guidelines may limit the diversity of the dataset; however, some of these constraints have the purpose of generating a dataset that reflects the multimodal nature of the dataset, without adding additional complexity (i.e., dealing with multiparty conversations). 

- The algorithm used for automatic punctuation restoration does introduce some degree of error, but this error is small enough so as not to affect the subsequent text processing steps. In the future, we are also planning to experiment with low dimensional representations such as word embeddings that do not rely on punctuation. 


==> reviewsICMI.tex <==
reviewer 1 review
score 4/5

  Rating

    Probably accept: I would argue for accepting this paper.

  Relevance to the ICMI

    Relevant

  Clarity

    Understandable by most readers

  Originality

    Quite creative

  Soundness

    Reasonable

  The Review

    Authors aim to classify medical videos on youtube on basis of the misinformation
    shared in the video. They used linguistic features (using words) , acoustic
    features (like pitch, pauses, jitters) and user engagement features for the
    developing this model.

    Positive:-
    - Very reasonable approach
    - Using publically available data
    - using well-known artifacts like DISCERN and PEMAT 

    Negative:-
    1. using accuracy to report in introduction. Because the dataset is not balanced,
    I would argue to not report this number here in the camera ready section
    2. Need more explanation on why a particular model was selected eg.
    2.1. why Bi LSTM ? was anything else tried?
    2.2. why linear SVM, anything else was tried?
    3. In section 3, criteria say not more than two speakers. In my opinion, even two
    people may be too much to handle. How many of the videos had two speakers?
    4. Video / Image features were not used at all.

  Questions to authors

    Reasonable approaches. Please replace the accuracy metric in the introduction as
    it may be misleading in unbalanced dataset.

  Comments after authors'  rebuttal

    (blank)

We will replace the accuracy metric with error reduction rate so it reflects more accurately the performance gain while using the proposed method. 

We selected an SVM classifier due to the limited number of examples and the large number of features. SVM classifiers have shown good performance in multimodal tasks in the past. We did try other algorithms, however they did not perform better than the SVM classifier. In addition, due to the limited training data we were unable to apply successfully a deep learning based model.
----------------------------------------------------------------

reviewer 2 review
score 4/5

  Rating

    Probably accept: I would argue for accepting this paper.

  Relevance to the ICMI

    Relevant

  Clarity

    Understandable by most readers

  Originality

    Quite creative

  Soundness

    Reasonable

  The Review

    (blank)

  Questions to authors

    (blank)

  Comments after authors'  rebuttal

    (blank)

----------------------------------------------------------------

reviewer 3 review
score 4/5

  Rating

    Probably accept: I would argue for accepting this paper.

  Relevance to the ICMI

    Relevant

  Clarity

    Very clear

  Originality

    Quite creative

  Soundness

    Reasonable

  The Review

    The paper presents an approach for automatic detection of misinformation on online
    medical videos in YouTube videos with prostate cancer as target video example.

    Paper Strengths - 
    The authors do a reasonable job in describing the details of how the dataset was
    created and presents a clear data annotation procedure with sufficient details
    about the annotation process.


    Paper Weakness
    It would be useful to address the differences between authors work and reference 1
    of the paper - “A content analysis of YouTube videos related to prostate cancer”.
    The sample size of 250 videos seem very small to conclude whether authors results
    are reliable and whether it would be validated for the larger set of 600000
    prostate cancer videos as mentioned in the paper.
    Does the automatic punctuation generation change the meaning of what was said as
    part of the video? It would be useful to see analysis on this aspect as well.

The main difference between our work and the study presented in reference 1 is that they only present descriptive and statistical analyses of the content of videos discussing prostate cancer that revealed the increasing presence of misinformative content. We present a data-driven approach that build models able to distinguish between the trustworthy and misinformative content in prostate cancer videos.

  Questions to authors

    How well does your method generalize to the full sample size on YouTube videos? 
    What is the scientific basis behind filtering procedure applied for the initial
    set collected to narrow down to 250 videos? For example, 5th point - video should
    not contain more than two speakers seems redundant filtering step when considering
    this task and limits the diversity of the dataset collected.

Since the quantity of videos in YouTube is constantly growing, it is difficult to say how our methods will generalize to the population of YouTube videos on prostate cancer. This study is more a seminal attempt on improving integrity of health-related online videos than a fully developed product. Our future research considers expanding our data collection to analyze a larger sample and confirm our findings. 

Our data collection guidelines are inspired in previous work that have analyzed the content of prostate cancer videos. As mentioned on the discussion section, we agree that some of the guidelines limit the diversity of the dataset; however, some of these constrains have the purpose of generating a dataset that reflects the multimodal nature of the dataset, without adding additional complexity (i.e., dealing with multiparty conversations). So future research can focus on studying the multimodal properties of misinformative content instead of preprocessing challenges. 

  Comments after authors'  rebuttal

    (blank)
